Unanimous Prediction for 100% Precision with Application to Learning Semantic Mappings

Can we train a system that, on any new input, either says "don't know" or makes a prediction that is guaranteed to be correct? We answer the question in the affirmative provided our model family is well-specified. Specifically, we introduce the unanimity principle: only predict when all models consistent with the training data predict the same output. We operationalize this principle for semantic parsing, the task of mapping utterances to logical forms. We develop a simple, efficient method that reasons over the infinite set of all consistent models by only checking two of the models. We prove that our method obtains 100% precision even with a modest amount of training data from a possibly adversarial distribution. Empirically, we demonstrate the effectiveness of our approach on the standard GeoQuery dataset.

==> Unique_mapping_ordering.tex <==
\begin{table}
	\begin{center}
		\scalebox{0.75}{
		\begin{tabular}{|c|c|}
			\hline
	\bf sentences 	 & \bf logical forms \\ \hline
	\nl{bag of Alex} & \wl{owner(Alex, bag)}\\ \hline
	\nl{Alex 's bag} & \wl{owner(Alex, bag)}\\ \hline
	\end{tabular}}
	\end{center}
		\caption{\label{unique_mappings_ordering} An example that shows we can conclude ordering form examples and uniqe mapping.
		From these examples we conclude: $M(\SF('s)) = \wl{owner(L,R)}$ while $M(\SF('s)) = \wl{owner(R,L)}$} where L and R means argument is in the left and right respectively.
\end{table}

==> approach.tex <==
\section{Approach}

We propose a method.


==> combination_example.tex <==
	\begin{figure}

	\scalebox{0.7}{
		\centering
	\begin{tabular}{cccccccc}

		&&&$M$(\nl{area}, \nl{of}, \nl{Ohio}) &&& \\
		\pause
		&&&\textdownarrow&&&\\
		
		$M$(&\{\nl{area}, \nl{of}, \nl{Iowa}\} &-& 
		\{\nl{cities}, \nl{in}, \nl{Iowa}\} &+& 
		\{\nl{cities}, \nl{in}, \nl{Ohio}\} &) \\
		\pause
		
				&&&\textdownarrow&&&\\
				
		&$M$(\{\nl{area}, \nl{of}, \nl{Iowa}\}) &-& 
		$M$(\{\nl{cities}, \nl{in}, \nl{Iowa}\}) &+& 
		$M$(\{\nl{cities}, \nl{in}, \nl{Ohio}\}) & \\
		\pause
				&&&\textdownarrow&&&\\
				
		& \{\wl{area}, \wl{IA}\} &-& 
		\{\wl{city}, \wl{IA}\} &+& 
		\{\wl{city}, \wl{OH}\} &&\\
		\pause
				&&&\textdownarrow&&&\\
				
		&&&\{\wl{area}, \wl{OH}\}&&&\\

	\end{tabular}}
	\caption{\label{fig:linear_combination}
		We predict the target atoms for the utterance \nl{area of Ohio} by adding and subtracting training inputs.
	}
	\end{figure}

==> context.tex <==

\subsection{Choosing source atoms}
\label{sec:context}
\input{table_consistent_inconsistent_merged.tex}
Our standing assumption is that each source atom maps to a multiset of target atoms in a context-independent way.
Due to polysemy, we cannot model source atoms simply as words;
but rather as $k$-grams.
In Table~\ref{tab:unigrams_and_bigrams},
if we use unigrams as source atoms, then equation $SM=T$ has no solution.
This is because word \nl{largest} is polysemous (can map to two different predicates).
If we use bigrams for source atoms, then $SM=T$ becomes consistent again.



==> context_result.tex <==
 \begin{table*}
 	\begin{center}
 		\begin{tabular}{|l|l|l|l|l|l|}
 			\hline   result/n-grams&  one-gram &  two-gram &  three-gram & four-gram & five gram \\ \hline
 			
 			{new source atoms} & 34 & 121 & 189 & 234 & 248\\ \hline
 			
 			{new target atoms} & 26 & 26 & 26 & 26 & 26\\ \hline
 			
 			{not in the row space} & 238 & 158 & 40 & 29 & 24\\ \hline
 			
 			{wrong answers} & 0 & 0 & 3 & 0 & 0\\ \hline
 			
 			{correct answers} & 0 & 0 & 47 & 16 & 8\\
 			\hline
 			
 			\bf{precision} & 0\% & 0\% & 94\% & 100\% & 100\%\\
 			\hline
 			
 			\bf{Recall} & 0\% & 0\% & 0.17\% & 0.06\% & 0.03\%\\
 			\hline
 		\end{tabular}
 	\end{center}
 	\caption{results!!!\label{context_result_wrong}}
 \end{table*}

==> experiments2.tex <==
\section{Experiments:}
\label{sec:experiments}
\input{goequery_stats}
We evaluate our approach on the standard GeoQuery dataset from \citet{zelle96geoquery},
which contains 880 utterances and their corresponding logical forms.
We use the variable-free functional logical form in \citep{kwiatkowski11lex} (See Figure~\ref{tab:compositional_target_atoms} for  examples).
We removed noisy and inconsistent examples by first minimizing $\|SM-T\|_1$ and then remove any example (row) with nonzero error.
We use the standard 600/280 train/test split \citep{zettlemoyer05ccg}.
See Table~\ref{tab:geo_stats} for statistics of Geoquery.
    
\input{experiments/precision_recall_numExample_curve}
We did all our experiments in the relax version of consistent mappings ($\sC^+$) which takes a few second to train and test.
We compute partial recovery recall for sentence $x$ as follows: $\frac{|M^*(x) \cap \hat{M}(x)|}{|M^*(x)|} * 100$ and average over all test sentences.

Figure~\ref{fig:number_of_examples_percentage_recovery} shows numbers of examples and their percentage of recovery. We partially recover 80\% of the data and fully recovered bag of predicates for 70\% of data.

\input{experiments/context_histogram.tex}
Figure~\ref{fig:precision_recall_numExample_curve} shows recall when we are interested in full recovery of bag of predicates.
As you see the precision is always 100\% no matter how many training examples we have and recall increases monotonically.

\input{experiments/experiment_with_only_one_point.tex}
\paragraph{Comparison with point estimation:}
We find an $M$ such that it minimizes $\|SM-T\|_2$, then for any $x$ in input we compute $y=xM$.
For a specific threshold ($\epsilon$)  if $[y_i-\epsilon, y_i+\epsilon)$ contains an integer we set $y_i$ to that integer otherwise we report ``don't know'' for predicate $i$.
We set $\epsilon$ to $\{0.1, 0.2, \dots, 0.5\}$ and plot precision recall curve.
You can see comparison between our algorithm and point estimation for half and all the training data in Figure~\ref{fig:experiment_with_only_one_point}.

    
\input{experiments/partial_mapping.tex}
\paragraph{Finding spans}
As stated we can find set of safe phrases so for every sentence we can go over all of its spans and check if its spans is in safe phrases Figure~\ref{fig:finding_spans} shows some spans that are in safe phrases.

\paragraph{Reconstructing of logical forms}
We choose target atoms to be variable free predicates (Figure~\ref{tab:compositional_target_atoms}) which helps reconstruction of logical forms.
As stated we can fully recover 70\% of testing examples in Geo. We use the method explained in Section~\ref{sec:ordering} and realized that 86\% of them can be uniquely reconstructed.

\input{experiments/recull_curve.tex}
\paragraph{Active Learning:}
Figure~\ref{Recall_numExample_curve_bag} shows the recall(recover the whole bag of predicate) when we choose examples randomly in comparison to when we choose examples using active learning.
We find that the latter requires half as many annotated logical forms as the former.

==> gaussian_elimination.tex <==
\begin{figure}[ht]
\begin{center}
\newcommand{\scc}{0.65}
\newcommand{\matindex}[1]{\mbox{\scriptsize#1}}
\newcommand{\matindexw}[1]{\mbox{\begin{sideways}\scriptsize#1\end{sideways}}}
\newcommand\sdw[1]{\begin{sideways}#1\end{sideways}}
\begin{tikzpicture}[scale=\scc]

		\node[scale=\scc] (S) at (0,0) { $\overbrace{\begin{blockarray}{ccccccc}
		&\matindex{\sdw{\nl{area}}} & \matindex{\sdw{\nl{Ohio}}} & \matindex{\sdw{\nl{cities}}} & \matindex{\sdw{\nl{of}}} & \matindex{\sdw{\nl{in}}} & \matindex{\sdw{\nl{Iowa}}}\\	
		\begin{block}{c[ccc|ccc]}
		\rightarrow & 1 & 0 & 0 & 1 & 0 & 1 \\
		\rightarrow & 0 & 1 & 0 & 0 & 0 & -1 \\ 
		& 0 & 0 & 1 & 0 & 1 & 1 \\
		\end{block}
		\end{blockarray}}^{\SF'}$};


		\node[scale=\scc] (T) at (6,0) { $\overbrace{\begin{blockarray}{cccc}
		\matindexw{\wl{area}} & \matindexw{\wl{city}} & \matindexw{\wl{OH}} & \matindexw{\wl{IA}} \\	
		\begin{block}{[cccc]}
		 1 & 0 & 0 & 1 \\
		 0 & 0 & 1 & -1 \\ 
		 0 & 1 & 0 & 1 \\
		\end{block}
		\end{blockarray}}^{\TF'}$};

	\end{tikzpicture}
\end{center}
\caption{\label{fig:gaussian_elimination}
$S'$ and $T'$ for our running examples after Gaussian elimination.
To compute $y$ for \nl{area of Ohio}, we add the first two rows of $S'$ and
check if it is equal to $x$.
In this case, it is, so we compute $y$ by adding first two rows of $T'$.}
\end{figure}	


==> geoquery_stats.tex <==
\begin{table}[t]
\begin{center}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|}
\hline
                        & \# words    & \# predicates & \# bigrams   \\ \hline
Training                & 249 / 153   & 146 / 54      & 866 / 582    \\ \hline
Training and Testing    & 282 / 172   & 165 / 57      & 1064 / 690   \\ \hline
\end{tabular}}
\caption{\label{tab:geo_stats} Statistics of Geoquery dataset before / after
  removing entity names based on the standard entity lexicon (e.g., $\nl{Seattle} \mapsto \wl{SEA}$).}
\end{center}
\end{table}


==> linear_combination.tex <==
\begin{figure*}
	\scalebox{0.7}{
		\centering
	\begin{tabular}{ccccccccccc}

		$M$(\nl{area}, \nl{of}, \nl{Ohio}) &=& $M$(&\{\nl{area}, \nl{of}, \nl{Iowa}\} &-& 
		\{\nl{cities}, \nl{in}, \nl{Iowa}\} &+& 
		\{\nl{cities}, \nl{in}, \nl{Ohio}\} &) &= \\
		
		&&& $M$(\{\nl{area}, \nl{of}, \nl{Iowa}\}) &-& 
		$M$(\{\nl{cities}, \nl{in}, \nl{Iowa}\}) &+& 
		$M$(\{\nl{cities}, \nl{in}, \nl{Ohio}\}) &&=& \\
		
		&&& \{\wl{area}, \wl{IA}\} &-& 
		\{\wl{city}, \wl{IA}\} &+& 
		\{\wl{city}, \wl{OH}\} &&=& 
		\{\wl{area}, \wl{OH}\}\\

	\end{tabular}}
	\caption{\label{fig:linear_combination}
    We predict the target atoms for the utterance \nl{area of Ohio} by adding and subtracting training inputs.

}
\end{figure*}


==> matrices_unique_answer.tex <==
\begin{figure*}[!ht]
	\newcommand{\matindex}[1]{\mbox{\scriptsize#1}}
	\begin{center}
		\scalebox{0.65}{$
			\overbrace{\begin{blockarray}{cccccc}
			\matindex{\nl{area}} & \matindex{\nl{of}} & \matindex{\nl{Ohio}} & \matindex{\nl{cities}} & \matindex{\nl{in}} & \matindex{\nl{Iowa}}\\	
			\begin{block}{[cccccc]}
			1 & 1 & 0 & 0 & 0 & 1 \\
			0 & 0 & 1 & 1 & 1 & 0 \\
			0 & 0 & 0 & 1 & 1 & 1 \\
			1 & 1 & 1 & 1 & 1 & 0 \\
			1 & 2 & 0 & 1 & 0 & 1 \\
			0 & 0 & 1 & 1 & 0 & 0 \\
			\end{block}
			\end{blockarray}}^{\SF} \times M = 			
			\overbrace{\begin{blockarray}{cccc}
			\matindex{\wl{area}} & \matindex{\wl{city}} & \matindex{\wl{OH}} & \matindex{\wl{IA}}\\	
			\begin{block}{[cccc]}
			1 & 0 & 0 & 1\\
			0 & 1 & 1 & 0\\
			0 & 1 & 0 & 1\\
			1 & 1 & 1 & 0\\
			1 & 1 & 0 & 1\\
			0 & 1 & 1 & 0\\
			\end{block}
			\end{blockarray}}^{\TF}\hspace{0.75cm}\implies\hspace{0.75cm}
			M=\begin{blockarray}{ccccc}
			&\matindex{\wl{area}} & \matindex{\wl{city}} & \matindex{\wl{OH}} &  \matindex{\wl{IA}}\\	
			\begin{block}{c[cccc]}
			\matindex{\nl{area}}		& 1 & 0 & 0 & 0\\
			\matindex{\nl{of}} 		& 0 & 0 & 0 & 0\\
			\matindex{\nl{Ohio}}		& 0 & 0 & 1 & 0 \\
			\matindex{\nl{cities}}	& 0 & 1 & 0 & 0 \\
			\matindex{\nl{in}}		& 0 & 0 & 0 & 0\\
			\matindex{\nl{Iowa}}		& 0 & 0 & 0 & 1\\
			\end{block}
			\end{blockarray}
			$}	
	\end{center}	
  \caption{\label{unique_answer} An example 
    where the linear system $\SF M = \TF$ has a unique solution.
  }
\end{figure*}


==> multiple_mappings_ordering.tex <==
\begin{table}
	\begin{center}
				\scalebox{0.75}{
		\begin{tabular}{|c|c|}
			\hline
	\bf sentences 		& \bf logical forms \\ \hline
	\nl{bag of Alex} 	& \wl{owner(Alex, bag)}\\ \hline
	\nl{bag} 			& \wl{bag}\\ \hline
	\nl{Alex} 			& \wl{Alex}\\ \hline
	\nl{light of bike}	& \wl{owner(bicycle, light)}\\ \hline
	\end{tabular}}
	\end{center}
	\caption{\label{multiple_mappings_ordering} An example that shows understanding ordering can lead to a unique mapping.}
\end{table}

==> note.tex <==
why 100\% precision 

Intro: explain more exmaple ra


too many extension emphasis that it is expendable

==> ordering.tex <==



 	\subsection{Reconstructing logical forms}
\input{compositional_target_atoms}
 	\label{sec:ordering}
While we have focused primarily on mapping to predicates,
we can reconstruct logical forms from the predicates.
As a preprocessing step,
we go over all the logical forms in the training examples.
We deem two predicates to be compatible if one comes as an argument of the other.
At test time, we search over all possible compatible ways of combining predicates into logical forms.
If there is exactly one, then we return that logical form and abstain otherwise.

To improve recall, we can define target atoms that include more information than just the predicates.
For example, we can conjoin the predicate with its parent,
its arguments order, etc.---see Figure~\ref{tab:compositional_target_atoms} for an example.
Note that more complex target atoms require more complex source atoms ($k$-grams) to realize
the modeling assumptions---that each source atom always maps to the same set of target atoms.
Thus, more data is required to estimate the additional parameters.

 	



==> paraphrase_examples.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\bf phrase & \bf paraphrase\\ \hline
\nlq{what are major} & \nlq{show major}\\
\nlq{states adjoin} & \nlq{states near}\\
\nlq{capital of} & \nlq{capital city of}\\
\nlq{people stay in} & \nlq{people in}\\ \hline
\end{tabular}
\end{center}
\caption{\label{tab:paraphrase_examples} Some examples of inferred paraphrases from Geoquery dataset}
\end{table}

==> partial_recovery.tex <==
\subsection{Partial semantic mappings}
\label{sec:partial_mapping}
\input{partial_recovery_running_examples}
\label{sec:partial_recovery}
Having new word or new combination of words is inevitable in natural language interfaces. In this section we answer this question: how much
of an utterance can we predict subject to 100\% precision?
In our running example (Figure~\ref{fig:sound_parser}), we have three training
inputs and there are only four different mappings
consistent with them (Figure~\ref{fig:atoms_and_mappings}). 
We do not know which one is the correct mapping,
but for some phrases such as: \nl{area of}, \nl{cities in}, \nl{Ohio}, and \nl{Iowa},
all four mappings unanimously agree.
Therefore, we can annotate any of these safe phrases that show up in any utterance.

Given a new utterance $x$,
we enumerate all of $x$'s contiguous phrases $r$
in increasing size and check if $r$ is in $\sFls$,
annotating $r$ with $\ourM(r)$ if it is.
Figure~\ref{fig:partial_recovery_running_examples}
shows how the algorithm treats unseen word or unseen combinations.
\fk{do u think I should explain that we have partial semantic mapping just because $M_{ij} \ge 0$}



==> tableSourceTargetAtoms.tex <==
\begin{figure*}
\begin{center}

		$\overbrace{\begin{blockarray}{lcccccc}
		&\matindex{\nl{area}} & \matindex{\nl{of}} & \matindex{\nl{Ohio}} & \matindex{\nl{cities}} & \matindex{\nl{in}} & \matindex{\nl{Iowa}}\\	
		\begin{block}{l[cccccc]}
		\matindex{\nl{area of Iowa}} & 1 & 1 & 0 & 0 & 0 & 1 \\
		\matindex{\nl{cities in Ohio}} & 0 & 0 & 1 & 1 & 1 & 0 \\
		\matindex{\nl{cities in Iowa}} & 0 & 0 & 0 & 1 & 1 & 1 \\
		\end{block}
		\end{blockarray}}^{S}$
		\hspace{1cm}
		$\overbrace{\begin{blockarray}{lcccc}
		&\matindex{\wl{area}} & \matindex{\wl{city}} & \matindex{\wl{OH}} & \matindex{\wl{IA}}\\	
		\begin{block}{l[cccc]}
		\matindex{\wl{area(IA)}} & 1 & 0 & 0 & 1\\
		\matindex{\wl{city(OH)}} & 0 & 1 & 1 & 0\\
		\matindex{\wl{city(IA)}} & 0 & 1 & 0 & 1\\
		\end{block}
		\end{blockarray}}^{T}
		$
\end{center}
\caption{\label{fig:SandT} matrix format of $S$ and $T$.}	
\end{figure*}

==> table_consistent_inconsistent_merged.tex <==
\begin{table*}[t]	
	\begin{center}
			\begin{tabular}{ccccc}
			\bottomrule 
 			\bf utterance & $\mathbf x_i$ (bigrams) & $\mathbf x_i$ (unigrams)& \bf logical form & $\mathbf y_i$\\ \hline
			\nl{largest city} &  [1,1,1,0,0,0,0,0] & [1,0,1,0]& \small\wl{largest(city)} & [1,0,0,1,0]\\ \hline

			\nl{largest river} & [1,0,0,1,1,0,0,0] & [1,0,0,1]& \small\wl{longest(river)} & [0,1,0,0,1]\\ \hline

			\nl{polluted city} & [0,0,1,0,0,1,1,0] & [0,1,1,0]& \small\wl{polluted(city)} & [0,0,1,1,0]\\ \hline

			\nl{polluted river}& [0,0,0,0,1,1,0,1] & [0,1,0,1] & \small\wl{polluted(river)} & [0,0,1,0,1]\\ \bottomrule



			\multicolumn{5}{l}{\small bigram source atoms=[\nl{\nothing\sep largest}, \nl{largest\sep city}, \nl{city\sep \nothing}, \nl{largest\sep river}, \nl{river\sep \nothing}, \nl{\nothing\sep polluted}, \nl{polluted\sep city}, \nl{polluted\sep river}]}\\

			\multicolumn{5}{l}{\small unigram source atoms=[\nl{largest}, \nl{polluted}, \nl{city}, \nl{river}]}\\  


			\multicolumn{5}{l}{\small target atoms=[\wl{largest}, \wl{longest}, \wl{polluted}, \wl{city}, \wl{river}]}\\ \bottomrule		
			\end{tabular}
		\end{center}
    \caption{\label{tab:unigrams_and_bigrams}
      An example showing how using bigram source atoms produces a consistent mapping,
    while unigram source atoms do not.}
\end{table*}



==> table_consistent_source_atoms.tex <==
\begin{table}

 	\begin{center}
 		\scalebox{0.7}{
 		\begin{tabular}{llll}
 			\toprule 
 			\bf utterance & $\mathbf x_i$& \bf logical form & $\mathbf y_i$\\ \hline
 			\nl{largest city} & [1,0,1,0] & \small\wl{largest(city)} & [1,0,0,1,0]\\ \hline
 			\nl{largest river} & [1,0,0,1] & \small\wl{longest(river)} & [0,1,0,0,1]\\ \hline
 			\nl{polluted city} & [0,1,1,0] & \small\wl{polluted(city)} & [0,0,1,1,0]\\ \hline
 			\nl{polluted river} & [0,1,0,1] & \small\wl{polluted(city)} & [0,0,1,0,1]\\ \bottomrule	

 			\multicolumn{4}{l}{\small source atoms=[\nl{largest}, \nl{polluted}, \nl{city}, \nl{river}]}\\ 
 			\multicolumn{4}{l}{\small target atoms=[\wl{largest}, \wl{longest}, \wl{polluted}, \wl{city}, \wl{river}]}\\ \bottomrule			
 		\end{tabular}}
 	\end{center}
 	\caption{\label{inconsistent_training_examples} This is an example that shows choosing wrong source atoms will lead to no consistent mapping.}
 \end{table}


==> table_inconsistent_source_atoms.tex <==

	
\begin{table}	
	\begin{center}
		\scalebox{0.65}{
			\begin{tabular}{llll}
			\bottomrule 
 			\bf utterance & $\mathbf x_i$& \bf logical form & $\mathbf y_i$\\ \hline
			\nl{largest city} &  [1,1,1,0,0,0,0,0,0] & \small\wl{largest(city)} & [1,0,0,1,0]\\ \hline
			\nl{largest river} & [1,0,0,1,1,0,0,0,0] & \small\wl{longest(river)} & [0,1,0,0,1]\\ \hline
			\nl{polluted city} & [0,0,1,0,0,1,1,0,0] & \small\wl{polluted(city)} & [0,0,1,1,0]\\ \hline
			\nl{polluted river}& [0,0,0,0,1,1,0,1,0] & \small\wl{polluted(river)} & [0,0,1,0,1]\\ \bottomrule


			\multicolumn{4}{p{10.5cm}}{\small source atoms=[\nl{\nothing\sep largest}, \nl{largest\sep city}, \nl{city\sep \nothing}, \nl{largest\sep river}, \nl{river\sep \nothing}, \nl{\nothing\sep polluted}, \nl{polluted\sep city}, \nl{polluted\sep river}, \nl{\nothing\sep city}]}\\ 
			\multicolumn{4}{l}{\small target atoms=[\wl{largest}, \wl{longest}, \wl{polluted}, \wl{city}, \wl{river}]}\\ \bottomrule		
			\end{tabular}}
		\end{center}
    \caption{\label{consistent_training_examples}
      An example showing how using bigram source atoms produces a consistent mapping,
    where unigram source atoms would not.}
\end{table}



==> two_different_mapping.tex <==
\begin{table}[ht]
	\begin{center}
	\scalebox{0.7}{
\begin{tabular}{|l|l|}
	\hline \bf mapping 1  & \bf mapping 2\\ \hline
	M(\nl{\nothing\sep largest}) =  \{\wl{}\} &
	M(\nl{\nothing\sep largest}) =  \{\wl{}\}\\
	
	M(\nl{largest\sep city}) =  \{\small\wl{largest}\} &
	M(\nl{largest\sep city}) =  \{\small\wl{largest}\}\\
	
	M(\nl{city\sep\nothing}) =  \{\small\wl{city}\} & 
	M(\nl{city\sep\nothing}) =  \{\wl{city}\}\\
	
	M(\nl{largest\sep river}) = \{\small\wl{longest}\} & 
	M(\nl{largest\sep river}) = \{\wl{longest}\}\\
	


	
	M(\nl{river\sep\nothing}) = \{\small\wl{river}\} & 
	M(\nl{river\sep\nothing}) = \{\small\wl{river}\}\\
	


	
	M(\nl{\nothing\sep polluted}) = \{\small\wl{polluted}\} & 
	M(\nl{\nothing\sep polluted}) = \{\wl{}\}\\
	
	M(\nl{polluted\sep city}) = \{\wl{}\} & 
	M(\nl{polluted\sep city}) = \{\small\wl{polluted}\}\\
	
	M(\nl{polluted\sep river}) =\{\wl{}\} & 
	M(\nl{polluted\sep river}) =\{\small\wl{polluted}\}\\
	\hline
\end{tabular}}
\end{center}
\caption{\label{two_different_mappings} Two different consistent mappings for Table~\ref{tab:unigrams_and_bigrams}.}
\end{table}

